Performance and Energy Optimization of Matrix Multiplication on Asymmetric big.LITTLE Processors

Asymmetric processors have emerged as an appealing technology for severely energy-constrained environments, especially in the mobile market where heterogeneity in applications is mainstream. In addition, given the growing interest on ultra low-power architectures for high performance computing, this type of platforms are also being investigated in the road towards the implementation of energy- efficient high-performance scientific applications. In this paper, we propose a first step towards a complete implementation of the BLAS interface adapted to asymmetric ARM big.LITTLE processors, analyzing the trade-offs between performance and energy efficiency when compared to existing homogeneous (symmetric) multi-threaded BLAS implementations. Our experimental results reveal important gains in performance while maintaining the energy efficiency of homogeneous solutions by efficiently exploiting all the resources of the asymmetric processor.

==> Olds/s5.1-one_kind_of_core.tex <==
The goal of the performance and energy efficiency tests in this section is to carry out 
an experimental study of both metrics comparing
the original multi-threaded of \gemm in BLIS against our asymmetric-aware implementation.
%
%The tests performed on the ODROID-XU3 allowed us to check the performance and the power consumption of the different CPU cores when working all together and also when running 
%independently. 
In all tests, we ensure the cores 
run at their highest frequency by setting the {\em performance} governor. 
Codes are instrumented with the {\tt pmlib}~\cite{AlonsoICPP12} framework, which 
collects power consumption data corresponding 
to instantaneous power readings from four independent sensors in the board 
(for the Cortex-A7 cores, Cortex-A15 cores, DRAM and GPU),
with a frequency of 200 ms$^{-1}$.

The first round of experiments analyzes the performance and energy behavior 
of the Cortex-A7 and the Cortex-A15 core types when working in isolation. For this purpose,
we execute a collection of \gemm kernels using one of the fine-grain paralelization 
exposed in Section~\ref{sec:performance}. Concretely, as the L2 cache
is shared among the cores of a cluster, we parallelize Loop~4 
using 1, 2, 3 and 4 threads (cores), with the performance and energy results
in Figure~\ref{fig:GFLOPS}. These plots reveal that the Cortex-A15 cores 
clearly deliver higher performance, with a rough increase of 2.5 GFLOPS per core, 
attaining a peak performance of about $10.2$ GFLOPS with 4 threads. 
For the Cortex-A7 cores, the 
performance peaks around $2.0$ GFLOPS and is also attained with 4~cores. 
Regarding energy efficiency, the Cortex-A15 obtains 
the best results in terms of GFLOPS/W. However, the benefits from
increasing the number of threads in this case are less significant (0.055 GFLOPS/W per core) 
when compared with those obtained with the Cortex-A7 cores (0.193 GFLOPS/W per core). 
It is also worth emphasizing that the use of 4 Cortex-A7 cores is more energy-efficient 
than an alternative that leverages a single Cortex-A15 core, though the overall 
performance of the former is slightly worse.

\begin{figure}[!ht]
\label{fig:GFLOPS}
\includegraphics[width=\columnwidth,height=5cm]{Plots/Data/dgemm_BLIS_GFLOPS_detail.pdf}
\includegraphics[width=\columnwidth,height=5cm]{Plots/Data/dgemm_BLIS_GFLOPSW_detail.pdf}
\caption{Performance (top) and energy efficiency (bottom) of the BLIS DGEMM using 
         exclusively one type of core, for a varying number of threads.}
\end{figure}


==> Olds/s5.2-asymmetric.tex <==
The second round of experiments 
evaluates the performance and energy efficiency of the asymmetric-aware port of BLIS to the 
big.LITTLE architecture. For this purpose,
we run a collection of \gemm kernels, 
relaying on a 2-way parallelization to distribute iterations of Loop~3
(see Section \ref{sec:performance}),
with a ratio of 6:1, among the cores of the fast and slow clusters, and taking advantage of
the independet L2 cache per cluster in this manner.  
For the fine-grain parallelization, 4 threads are leveraged 
in order to assign chunks of the iteration space 
for Loop~4 to each core within the cluster. Our experiments with different
configurations revealed this option to be the most efficient 
for the target big.LITTLE architecture.

Figure~\ref{fig:AMP} reports the results for this second evaluation.
The line labeled as ``{big.LITTLE (4+4 threads)}'' 
corresponds to the asymmetric-aware implementation. 
The same \gemm kernels were computed with BLIS using a symmetric workload distribution 
(the iteration space is equally distributed among the Cortex-A7 and Cortex-A15 cores), 
with the results labelled as ``{A7+A15 (4+4 threads)}'' in the figure. 
For comparison purposes, the performance and energy obtained using exclusively 
four Cortex-A7 or four Cortex-A15 CPUs are also added. Finally, the ``ideal'' line
corresponds to the sum of the peak performances of the configurations 
that use four cores of each of the two types in isolation (i.e., the performance of the four
Cortex-A15 cores plus the performance of the four Cortex-A7 cores).

These performance results show that the AMP configuration 
outperforms the peak performance of all other configurations being close to the ideal case. 
The increment 
compared to the configuration that employs four Cortex-A15 cores for the largest tested problem
is close to 20\%. 
The asymmetric version does not outperform the original version for small matrices 
though, as the chunks assigned to the big and LITTLE cores are, in those cases, 
too small to exploit the asymmetric architecture.
%Note that, the workload distribution is set a priori taking into account the CPU's peak performance and not the \gemm performance. 
In terms of energy-efficiency, the AMP configuration is as efficient as the symmetric setup using 
exclusively four Cortex-A15 CPU.% but at the exchange of a significantly higher performance.

The symmetric workload distribution attains about 40\%
of the highest performance that is observed when employing only the Cortex-A15 cores. 
The reason is that, with the symmetric workload distribution, 
thread scheduling is delegated to the operating system or the
OpenMP runtime, using a homogeneous distribution of chunks. 
This causes a severe load imbalance as the fast Cortex-A15 
threads finish processing their assigned chunk, and have to wait a long time
for the Cortex-A7 threads to complete their assignment. 
The energy-efficiency is also affected,
and this configuration achieves the worst energy-efficiency.

\begin{figure}[!ht]
\includegraphics[width=\columnwidth,height=5cm]{Plots/Data/dgemm_BLIS_GFLOPS.pdf}
\includegraphics[width=\columnwidth,height=5cm]{Plots/Data/dgemm_BLIS_GFLOPSW.pdf}
\caption{\label{fig:AMP}Performance (top) and energy efficiency (bottom) of the BLIS DGEMM 
         implementations using a single as well as different types of cores.}
\end{figure}


==> s2-related.tex <==
%\section{Related Work}
%\label{sec:related}

Heterogeneous (and asymmetric) architectures are an active research topic,
with a vast design space which needs careful consideration in terms of power, performance, 
programmability, and flexibility~\cite{Chi12}. 
Basically, these works can be grouped into 
{\em i)} efforts to experimentally evaluate the
computational performance and/or power-energy efficiency of
AMPs using multithreaded benchmarks and applications; and 
{\em ii)} results related to workload-partitioning
strategies for the execution of \gemm on heterogeneous platforms.
%
In the first group, %Winter et al.~\cite{Win10} 
%discuss power management techniques and thread scheduling for AMPs;
%(indeed, 
scheduling on this AMP architectures is explored in a large number of works; see,
among many others, ~\cite{Hou09,Lak09,Rod13,Win10} and the references therein.
%
In the second group, how to map \gemm in an heterogeneous cluster has been analyzed
in~\cite{Cla11}, while a theoretical study of the performance of dynamic scheduling applied
to this kernel is introduced in~\cite{Bea14}. 

%Refer to 2D distribution of workload + matrix multiplication in Euro-Par...

Compared with previous works, our paper proposes a preliminar study of performance, energy efficiency and
 necessary mechanisms to be adopted in order to adapt a complete and professionally maintained open source BLAS library (BLIS)
to asymmetric ARM big.LITTLE architectures. Given that the complete BLIS library is heavily
based on the mechanics of the \gemm\ implementation, this is a necessary step towards the development
of the first complete BLAS implementation for asymmetric processors.

